Sublinear Algorithms for $(1.5+\epsilon)$-Approximate Matching

We study sublinear time algorithms for estimating the size of maximum matching. After a long line of research, the problem was finally settled by Behnezhad [FOCS'22], in the regime where one is willing to pay an approximation factor of $2$. Very recently, Behnezhad et al.[SODA'23] improved the approximation factor to $(2-\frac{1}{2^{O(1/\gamma)}})$ using $n^{1+\gamma}$ time. This improvement over the factor $2$ is, however, minuscule and they asked if even $1.99$-approximation is possible in $n^{2-\Omega(1)}$ time. We give a strong affirmative answer to this open problem by showing $(1.5+\epsilon)$-approximation algorithms that run in $n^{2-\Theta(\epsilon^{2})}$ time. Our approach is conceptually simple and diverges from all previous sublinear-time matching algorithms: we show a sublinear time algorithm for computing a variant of the edge-degree constrained subgraph (EDCS), a concept that has previously been exploited in dynamic [Bernstein Stein ICALP'15, SODA'16], distributed [Assadi et al. SODA'19] and streaming [Bernstein ICALP'20] settings, but never before in the sublinear setting. Independent work: Behnezhad, Roghani and Rubinstein [BRR'23] independently showed sublinear algorithms similar to our Theorem 1.2 in both adjacency list and matrix models. Furthermore, in [BRR'23], they show additional results on strictly better-than-1.5 approximate matching algorithms in both upper and lower bound sides.

==> 1-introduction.tex <==
\section{Introduction}
\thatchaphol{TODO: Check if there exists duclicate bib-item}


Computing a large matching in graphs is one of the cornerstones in graph algorithms. Numerous powerful techniques has been developed \textbf{CITE} towards almost-linear time algorithms. Recently, this is finally achieved in bipartite graphs Chen et al.~\cite{chen2022maximum} and remains open in general graphs. The next question is then to what extent can we compute a large matching in \emph{sublinear} time without reading the whole graph? It turns out that linear time is necessary to \emph{find} any $O(1)$-approximate maximum matching.\footnote{\textbf{TODO: }Show this.} Hence, the natural goal is to estimate the \emph{size} of the maximum matching. 

The next question is then to what extent can we compute a large matching in \emph{sublinear} time without reading the whole graph? It turns out that linear time is necessary to \emph{find} any $O(1)$-approximate maximum matching.\footnote{\textbf{TODO: }Show this.} Hence, the natural goal is to estimate the \emph{size} of the maximum matching. 

For the last 15 years, there has been an impressive line of work addressing this question. The model of the algorithms studied in the literature is as follows. Given an input graph $G=(V,E)$ with $n$ vertices that have maximum degree $\Delta$ and average degree $d$, the vertex set $V$ is known to the algorithm. In contrast, the algorithm can access the edge set $E$ either by making only \emph{adjacency-matrix queries}, or by making only \emph{adjacency-list queries}, as defined below. 
\begin{enumerate}
\item An \textbf{adjacency-matrix query} takes an unordered pair of vertices $\{u,v\}\in{V \choose 2}$, and returns whether $\{u,v\}\in E$.
\item An \textbf{adjacency-list query} takes an ordered pair $(v,i)$, where $v\in V$ and $i\in[n]$, and returns the $i^{th}$ edge incident on $v$ in $E$ or returns $\perp$ if $i\ge\deg_{G}(v)$.
\end{enumerate}
We also say that the algorithm has a \emph{matrix-access }or \emph{list-access }to the graph, respectively. Let $\mu(G)$ denote the size of the maximum matching of $G$. An $(\alpha,\beta)$-approximation algorithm returns an estimate $\tilde{\mu}$ where $\tilde{\mu}\le\mu(G)\le\alpha\tilde{\mu}+\beta$. 

Early work in this area focused on showing constant-time algorithms when $\Delta=O(1)$. A notable work by Yoshida~et~al.~\cite{yoshida2009improved} shows how to obtain a $(1,\epsilon n)$-approximation in $\Delta^{O(1/\epsilon^{2})}$ time with list-access. However, these early algorithms \cite{parnas2007approximating,nguyen2008constant,yoshida2009improved,onak2012near} may take $\Omega(n^{2})$ time in general graphs. It was until 2020 when sublinear algorithms on general graphs were shown. Sublinear time algorithms with $(O(1),\epsilon n)$-approximation was given by Kapralov et al.~\cite{kapralov2020space} and $(2,\epsilon n)$-approximation was given by Chen et al.~\cite{chen2020sublinear} (based on \cite{onak2012near}). These algorithms, however, are not optimal. See \Cref{tab:summary} for details.



\begin{table}
\footnotesize{

\begin{tabular}{|>{\raggedright}p{0.1\textwidth}|>{\centering}p{0.15\textwidth}|>{\centering}p{0.1\textwidth}|>{\centering}p{0.1\textwidth}|>{\centering}p{0.1\textwidth}|>{\centering}p{0.15\textwidth}|>{\centering}p{0.1\textwidth}|}
\hline 
Model & \multicolumn{2}{c|}{Adjacency List } & \multicolumn{2}{c|}{Adjacency List } & \multicolumn{2}{c|}{Adjacency Matrix}\tabularnewline
\hline 
Guarantee & Approx & Time & Approx & Time & Approx & Time\tabularnewline
\hline 
\hline 
\cite{parnas2007approximating} & $(2,\epsilon n)$ & $\Delta^{O(\log(\Delta/\epsilon)}$ &  &  &  & \tabularnewline
\hline 
\multirow{2}{0.1\textwidth}{\cite{nguyen2008constant}} & $(2,\epsilon n)$ & $2^{O(\Delta)}/\epsilon^{2}$ &  &  &  & \tabularnewline
\cline{2-7} 
 & $(1,\epsilon n)$ & $2^{\Delta^{O(1/\epsilon)}}$ &  &  &  & \tabularnewline
\hline 
\multirow{2}{0.1\textwidth}{\cite{yoshida2009improved}} & $(2,\epsilon n)$ & $\Delta^{4}/\epsilon^{2}$ &  &  &  & \tabularnewline
\cline{2-7} 
 & $(1,\epsilon n)$ & $\Delta^{O(1/\epsilon^{2})}$ &  &  &  & \tabularnewline
\hline 
\cite{onak2012near,chen2020sublinear} & $(2,\epsilon n)$ & $(d+1)\Delta/\epsilon^{2}$  &  &  & $(2,\epsilon n)$ & $n\sqrt{n}/\epsilon^{2}$ \tabularnewline
\hline 
\cite{kapralov2020space} & $(O(1),\epsilon n)$ & $\Delta/\epsilon^{2}$ & $O(1)$ & $n+\Delta^{2}/d$ &  & \tabularnewline
\hline 
\cite{behnezhad2022time} & $(2,\epsilon n)$ & $(d+1)/\epsilon^{2}$ & $2+\epsilon$ & $n+\Delta/\epsilon^{2}$ & $(2,\epsilon n)$ & $n/\epsilon^{3}$\tabularnewline
\hline 
\cite{behnezhad2023beating} & $(2-\frac{1}{2^{O(1/\gamma)}},o(n))$ & $(d+1)\Delta^{\gamma}$ & $2-\frac{1}{2^{O(1/\gamma)}}$ & $n+\Delta^{1+\gamma}$ & $(2-\frac{1}{2^{O(1/\gamma)}},o(n))$ & $n^{1+\gamma}$\tabularnewline
\hline 
\textbf{Ours} & $(1.5,\epsilon n)$ & $nd^{1-\Omega(\epsilon^{2})}$ & $1.5+\epsilon$ & $n\Delta^{1-\Omega(\epsilon^{2})}$ & $(1.5,\epsilon n)$ & $n^{2-\Omega(\epsilon^{2})}$\tabularnewline
\hline 
\end{tabular}

}

\caption{Summary of sublinear-time algorithms for estimating the size of maximum matching. We omit $\protect\polylog(n/\epsilon)$ factors. The results by \cite{onak2012near} had subtleties. They first claimed a $(2,\epsilon n)$-approximation algorithms with time $(d+1)/\protect\poly(\epsilon)$ in the adjacency list model and $n/\protect\poly(\epsilon)$ in the adjacency matrix model. We show their bounds after fixing by \cite{chen2020sublinear} instead.\label{tab:summary}}
\end{table}


Finally, Behnezhad \cite{behnezhad2022time} gave algorithms with near-optimal time when the approximation is around $2$. More precisely, with list access, he showed (i) a $(2,\epsilon n)$-approximation algorithm with $\Otil((d+1)/\epsilon^{2})$ time using list-access, (ii) a $(2+\epsilon)$-approximation algorithm with $\Otil(n/\epsilon^{2})$ time using list-access, and (iii) a $(2,\epsilon n)$-approximation algorithm with $\Otil(n/\epsilon^{3})$ time using matrix-access.\footnote{Behnezhad's result \cite{behnezhad2022time} are optimal because (i) any $(O(1),\epsilon n)$-approximation algorithms with $\Omega(d)$ adjacency list queries \cite{parnas2007approximating}, (ii) it requires $\Omega(n)$ adjacency list queries to distinguish whether an input graph contain an edge or is empty, (iii) it requires $\Omega(n)$ matrix adjacency matrix queries to distinguish whether an input graph is a perfect matching or is empty.} Very recently, Behnezhad et al.~\cite{behnezhad2023beating} showed that, for any constant $\gamma>0$, the factor of $2$ in all three results can be improved to $2-\frac{1}{2^{O(1/\gamma)}}$ by paying an additional factor of $\Delta^{\gamma}$ in time. This improvement over the factor $2$ is, however, minuscule and it was explicitly posted as an open problem in \cite{behnezhad2023beating} whether even $1.99$-approximation is possible in $n^{2-\Omega(1)}$ time.



\paragraph{Our Results.}
We give a strong affirmative answer to this open problem by showing the first sublinear algorithms with approximation factor close to $1.5$.
\begin{thm}
\label{thm:main}For any $\epsilon>0$, there are algorithms that, given a graph $G$, w.h.p. estimates the size of maximum matching up to
\begin{enumerate}
\item $(1.5+\epsilon)$-approximation in $\Otil(n\Delta^{1-\Omega(\epsilon^{2})})$ time using adjacency-list queries,
\item $(1.5,\epsilon n)$-approximation in $\Otil(nd^{1-\Omega(\epsilon^{2})})$ time using adjacency-list queries, and
\item $(1.5,\epsilon n)$-approximation in $n^{2-\Omega(\epsilon^{2})}$ time using using adjacency-matrix queries.
\end{enumerate}
\end{thm}



Our algorithms in \Cref{thm:main} make a significant step toward the ultimate goal of $(1,\epsilon n)$-approximation algorithms in sublinear time. Such algorithms would have impact beyond the area of sublinear algorithms. For example, a $(1,\epsilon n)$-approximation algorithm with $n^{2-\Omega(1)}$ time using using matrix-access would immediately imply the first fully dynamic algorithm that can $(1+\epsilon)$-approximate the size of maximum matching using $n^{1-\Omega(1)}$ update time, which is one of the biggest open problem area of dynamic graph algorithms. See, e.g.~\cite{bhattacharya2023dynamic}, for the reduction. 

\paragraph{Our Techniques.}
The technique behind \Cref{thm:main} diverges from all previous sublinear matching algorithms. In brief, we show how to exploit the \emph{edge-degree constrained subgraph} (EDCS) in the sublinear model. This object has been successfully used in dynamic algorithms \cite{bernstein2015fully,bernstein2016faster}, distributed algorithms \cite{assadi2019coresets}, streaming algorithms \cite{bernstein2020improved,assadi2021beating}, but never before in sublinear algorithms.

More specifically, we show that the variant of EDCS introduced in \cite{bernstein2020improved}, which we call \emph{edge-degree bounded subgraph} (EDBS), can be implemented in sublinear time. Once we identify the correct key object of our sublinear algorithm, the whole algorithms follows naturally and is conceptually very simple.

\paragraph{Remarks.}
Our technique reveals further interesting connections beyond our main result in \Cref{thm:main}. First, we show that our sublinear algorithms can be improved significantly using $(1,\epsilon n)$-approximation algorithms whose running time is \emph{not} sublinear. 
\begin{thm}
If there exists a $(1,\epsilon n)$-approximate matching algorithm with $\Otil_{\epsilon}(n\Delta^{c})$ time using matrix-access, then there exists a $(1.5,\epsilon n)$-approximate matching algorithm with $\Otil_{\epsilon}(n^{2-1/c})$ time using matrix-access.
\end{thm}

For example, we could obtain $(1.5,\epsilon n)$-approximation in $\Otil_{\epsilon}(n^{1.5})$ time if there exists a $(1,\epsilon n)$-approximation algorithm with $O_{\epsilon}(n\Delta)$ time. Note that $O(n\Delta)$ is not sublinear in $m$, the number of edges. Next, we show the following:
\begin{thm}
There is a algorithm with list-access to a graph $G$ and in time $\tilde{O}_{\epsilon}(n\cdot\Delta^{1-\Theta(\epsilon^{2})})$ returns w.h.p. either 
\begin{itemize}
\item an explicitly matching of size $\Omega(\epsilon\mu(G))$, or 
\item a $(1+\epsilon)$-approximation estimate of $\mu(G)$.
\end{itemize}
\end{thm}

This result is interesting because the first task alone is impossible in sublinear models, and the second task is still out-of-reach from the current techniques. \textbf{TODO: how to write it in a more excting way?}



==> 4-approximating_the_matching_size_in_H.tex <==

\section{Approximating the matching size in $H$}

\label{sec:approx-matching}

Note that this section is deduced from \cite{YoshidaYI12} in a straightforward manner.

\begin{lem}

\label{lm:approx-matching}

Given adjacency list access to the edges of graph $G$ with maximum degree $\Delta = O(n^{\delta})$ there is an algorithm which returns a $(1 + \epsilon)$-approximation to the maximum matching size of $G$ in $\tilde{O}\left(\frac{n^{1 + \delta/\epsilon^2}}{\mu(G)}\right)$ time.

\end{lem}

\begin{proof}

\cite{YoshidaYI12} showed the following: for graph $G = (V,E)$ there is a randomized algorithm which can determine the matched status of a uniformly randomly chosen vertex in $V$ under some $(1+\epsilon)$-approximate maximum matching $M_{1 + \epsilon}$ in expected $\tilde{O}(\Delta^{O(1/\epsilon^2)})$ time assuming the algorithm has adjacency list query access to $G$. We will refer to this result in a black-box manner. We will furthermore assume that we have access to a constant approximation of $\mu(G)$ (from \cite{Behnezhad21}).

The algorithm samples $T = \Omega(\frac{n \cdot \log(n)}{\mu(G) \cdot  \epsilon^2})$ vertices $V_T$ uniformly at random from $V$. For each vertex in $V_T$ the algorithm checks if they are matched under $M_{1 + \epsilon}$, call such vertices as $V_T'$. We will argue that $\frac{|V_T'|}{|V_T|} \cdot \frac{n}{2} \in \mu(G) \cdot (1 \pm O(\epsilon))$ with high probability. 

Let $x_i$ be the indicator variable of the event where the $i$-th sampled vertex in $V_T$ is matched under $M_{1 + \epsilon}$ and let $X = \sum x_i$. Observe, that $\E[x_i] = \frac{2 \cdot |M_{1+\epsilon}|}{n} \in \frac{2 \cdot \mu(G)}{n} \cdot (1 \pm O(\epsilon))$ and $x_i$ form independently distributed random variables. Using standard Chernoff bounds we get that:

\begin{eqnarray}
\Pr\left(\frac{|V_T'|}{|V_T|} \cdot \frac{n}{2} \notin \mu(G) \cdot (1 \pm O(\epsilon)) \right) & = & \Pr(X \notin \E[X] \cdot (1 \pm O(\epsilon))\nonumber \\
& \leq & \exp\left(-\Omega(\epsilon^2 \cdot \E[x_i] \cdot |V_T|)\right) \nonumber \\
& \leq & \exp(-\Omega(\log(n)))
\end{eqnarray}

Hence, $X \in \mu(G) \pm(1 + O(\epsilon))$ with high probability. This means if the algorithm simply returns a value of $X - \gamma \cdot \mu(G)$ for some constant $\gamma$ based on $\epsilon$ we get that $\mu(G) \cdot (1 - O(\epsilon)) \leq X - \gamma \cdot \mu(G) \leq \mu(G)$.

The running time of the algorithm is proportional to $\tilde{O}(|V_T| \cdot \Delta^{1/\epsilon^2}) = \tilde{O}(\frac{n^{1 + \delta/\epsilon^2}}{\mu(G)})$

\end{proof}

\subsection{Proof of Theorem~\ref{thm:main}}

For the case of adjacency list query access to the graph the theorem is a black-box combination of lemmas \ref{lm:core-subgraph:framework}, \ref{lm:generatingsubgraph:listqueries} and \ref{lm:approx-matching}. The total running time we receive this way is proportional to $\tilde{O}(n^{2-\delta} + \frac{n^{1 + \delta/\epsilon^2}}{\mu(G)} \cdot \frac{n^2}{\mu(G)}) = \tilde{O}(\frac{n^{3 + \delta/\epsilon^2}}{\mu(G)^2} + n^{2-\delta})$. Note that if $m \in O(n^{2-\delta})$ the statement is follows from standard static matching algorithms, and if $m \in \Omega(n^{2-\delta})$ then $\mu(G) \in \Omega(n^{1-\delta})$. Hence, assuming $\delta \in O(\epsilon^2)$ the algorithm has running time $\tilde{O}(n^{2-\Omega(\epsilon)^2})$.

For the case of adjacency matrix queries first note that we may assume that $\mu(G) \in \Omega_\epsilon(n)$ as argued in \cref{sec:prelims}. Hence black-box combination of lemmas \ref{lm:core-subgraph:framework}, \ref{lm:generatingsubgraph:matrixqueries} and \ref{lm:approx-matching} we get a running time of $\tilde{O}(n^{2-\Omega(\epsilon^2)})$ as long as $\delta \in O(\epsilon^2)$.

==> deleted_bits.tex <==
Focus on color $c \in \mathcal{C}$. We will sample $\frac{\bar{\mu} \cdot \log(n) \cdot 10}{n^\delta \cdot \epsilon^3}$ colors from $\mathcal{C}$, lets call the sample multiset $\mathcal{C}_c$. If and only if $|\{c' \in \mathcal{C}_c | (c,c') \in E_\mathcal{C} \land deg_H((c,c')) < \beta - 1\}| \geq 20 \cdot \log(n)$ we say that $c \in \mathcal{C}_D$. Observe, that to execute this sampling process for each color it takes $\tilde{O}(\frac{\bar{\mu}^2}{n^\delta})$ edge queries to $(\mathcal{C}, U_H)$ and hence $\tilde{O}(\frac{n^2}{\bar{\mu}^2} \cdot \frac{\bar{\mu}^2}{n^\delta}) = \tilde{O}(n^{2-\delta})$ queries to $G$. Furthermore, once $\mathcal{C}_D$ and $H$ is calculated an adjacency matrix query of $(\mathcal{C}, U_A)$ takes time proportional to an adjacency matrix query of graph $(\mathcal{C}, U_H)$. Hence, an adjacency list query of $U_H$ can be completed in $\tilde{O}(\frac{n^2}{\bar{\mu}^2} \cdot n)$ time. As argued in \Cref{sec:prelims} when talking about adjacency matrix queries of $G$ we may assume that $|V| \in O_\epsilon(\mu(G))$, hence this query time is upper bounded by $\tilde{O}(\frac{n^2}{\bar{\mu(G)}})$.

Now we have to argue about the correctness of the calculation of set $\mathcal{C}_D$. Fix a color $c$ and consider the color multiset $\mathcal{C}_c$. For some sample $c' \in \mathcal{C}_c$ the event where $(c,c')$ is in $E_\mathcal{C}$ and has degree lesser than $\beta - 1$ in $H$ is Bernoulli random variable with mean $\frac{deg_{U_H}(c)}{|\mathcal{C}|}$ independently from all other colors. For the $i$-th sample call the indicator variable of this event as $x_i$ and let $X = \sum x_i$. Assume that $deg_{U_H}(c) > \frac{n^\delta \cdot 4}{\epsilon^2}$, hence $\E[x_i] \geq \frac{4 \cdot \epsilon^2}{n^{1 - \delta}}$. Using standard Chernoff bounds we get that.

\begin{eqnarray}
\Pr\left(|\{c' \in \mathcal{C}_c | (c,c') \in E_\mathcal{C} \land deg_H((c,c')) < \beta - 1\}| < 10 \cdot \log(n) \right)  & = & P(X > 10 \cdot \log(n))\nonumber \\
\Pr(X < \E[X]/2) & \leq & \exp(-\frac{\E[X]}{8}) \nonumber \\
& \leq & \frac{1}{poly(n)} \nonumber
\end{eqnarray}

This implies that any color with degree at least $2 \cdot n^\delta/\epsilon^2$ in $U_H$ is in $\mathcal{C}_D$ with high probability. It remains to show that any color with degree at most $n^\delta/\epsilon^2$ in $\mathcal{C}$ is not in $\mathcal{C}$. Assume that $c$ is such a color. Then $\E[x_i] = \frac{deg_{U_H}(c)}{|\mathcal{C}|} \leq \frac{\epsilon^2 \cdot n^\delta}{|\mathcal{C}|}$. Similarly arguing based on Chernoff bounds we get the following lines of inequalities: 

\begin{eqnarray}
\Pr\left(|\{c' \in \mathcal{C}_c | (c,c') \in E_\mathcal{C} \land deg_H((c,c')) < \beta - 1\}| > 20 \cdot \log(n) \right)  & = & P(X > 20 \cdot \log(n))\nonumber \\
\Pr(X > 2 \cdot \E[X]) & \leq & \exp(-\frac{\E[X]}{3}) \nonumber \\
& \leq & \frac{1}{poly(n)} \nonumber
\end{eqnarray}

Hence, taking union bound over all colors we get that if $deg_{U_H}(c) < n^\delta/\epsilon^4$ then $c \notin \mathcal{C}$.
